Unleashing Unprivileged eBPF Potential with Dynamic Sandboxing

For safety reasons, unprivileged users today have only limited ways to customize the kernel through the extended Berkeley Packet Filter (eBPF). This is unfortunate, especially since the eBPF framework itself has seen an increase in scope over the years. We propose SandBPF, a software-based kernel isolation technique that dynamically sandboxes eBPF programs to allow unprivileged users to safely extend the kernel, unleashing eBPF's full potential. Our early proof-of-concept shows that SandBPF can effectively prevent exploits missed by eBPF's native safety mechanism (i.e., static verification) while incurring 0%-10% overhead on web server benchmarks.

==> background.tex <==

We introduce the concept of \ebpf and identify the weaknesses of its safety mechanism in~\S\ref{sec:background:ebpf}. 
In~\S\ref{sec:background:motivation}, we use a CVE to motivate the need for dynamic isolation of~\ebpf.

\subsection{\ebpf}
\label{sec:background:ebpf}

\begin{figure}
	\centering
	\includegraphics[width=0.7\columnwidth]{img/ebpf-workflow.png}
	\caption{An overview of the \ebpf workflow.}
	\label{fig:ebpf_workflow}
\end{figure}

eBPF is a Linux framework originally derived from the Berkeley Software Distribution (BSD) for executing packet filtering programs in the kernel.\footnote{Microsoft Windows' version of \ebpf is under development~\cite{windows_ebpf}.}
Today, eBPF is used not only for networking, but also for tracing~\cite{ply_tracing}, monitoring~\cite{pulsar_monitoring}, and security~\cite{kubearmor_security} purposes.

\subsubsection{\ebpf Workflow}
\autoref{fig:ebpf_workflow} shows the general workflow of \ebpf.
Developers can write \ebpf programs in C and compile them into \ebpf bytecode using a Clang compiler (for other languages, \eg Rust, Clang is replaced by the equivalent LLVM-based compiler).
To minimize the risks of running user-defined kernel extensions, the \ebpf verifier~(\S\ref{sec:background:ebpf:verifier}) statically verifies all \ebpf bytecode at load time.
Once the bytecode is verified, an architecture-specific Just-In-Time (JIT) compiler maps each bytecode to its corresponding native machine code, so the final \ebpf image can run as efficiently as natively compiled kernel code.
Before the JIT-compiled \ebpf image gets attached to its designated kernel hook point, where the \ebpf program gets triggered and executed at runtime, the \ebpf image is marked as read-only to prevent any corruptions throughout its lifetime.
\ebpf supports 43 types of hook points, with each \ebpf program type using at least one type of hook.
For example, kprobe hooks and Linux Security Module (LSM) hooks allow \ebpf programs to collect debugging information and mediate access to kernel objects, respectively.
During runtime, user space processes can interact with \ebpf programs via special shared data structures such as \ebpf~maps.


\subsubsection{\ebpf Verifier}
\label{sec:background:ebpf:verifier}
The \ebpf verifier performs a two-pass static verification on all \ebpf programs~\cite{ebpfverifier}.
The first pass is a depth-first search, where \ebpf programs that are either too large (exceed 4096 instructions) or contain unreachable instructions, unbounded loops, or out-of-bounds jumps, are rejected.
The second pass walks all instructions starting from the first instruction, simulating the execution of every instruction while tracking registers and stack states to catch unsafe operations.
On entry to each instruction, each register is assigned a type.
The simulation of instruction execution changes the types of the registers depending on instruction semantics.
For instance, the \ebpf verifier forbids pointer arithmetic.
The addition of two pointers results in a register state of type \texttt{SCALAR\_VALUE}, indicating that the register value is not a valid pointer.
Any instructions accessing the invalid pointer will be caught by the verifier at load time.

We briefly discuss the security policies enforced by the verifier on \emph{privileges} and \emph{\ebpf helper functions}. 
We also identify the limitations of the \ebpf verifier, which highlight the problem with static verification -- runtime security is not always guaranteed.

\smallskip
\noindgras{Privileges.}
\ebpf programs executed with \texttt{CAP\_BPF} or \texttt{CAP\_SYS\_ADMIN} capabilities are \emph{privileged} while those executed with a non-privileged user capability are \emph{unprivileged}.
Privileged \ebpf has full access to all features in \ebpf.
Due to security concerns over user-provided kernel extensions, unprivileged \ebpf is subject to a reduced set of functionality and restricted access to the kernel.
In particular, unprivileged users are allowed to use only 2 out of 32 types of \ebpf programs, thereby restricting the use case of unprivileged \ebpf to only socket filtering. 
To prevent unprivileged users from leaking sensitive kernel information, unprivileged \ebpf programs are not allowed to store kernel pointers in \ebpf maps, a data structure shared between \ebpf and user-space programs.

\smallskip
\noindgras{\ebpf Helper Functions.}
The \ebpf verifier ensures that \ebpf programs interact with the kernel only through a predefined allowlist of \ebpf helper functions.
The \ebpf helper functions forms a well-defined interface that mediates all interactions between \ebpf programs and the kernel.
For example, an \ebpf program has to call the \texttt{bpf\_get\_current\_task} helper function, which performs the kernel operation on its behalf, to get the pointer to the current task.
The \ebpf helper functions are part of the core kernel and they cannot be extended or modified without recompiling the kernel.

\smallskip
\noindgras{Limitations.}
The \ebpf verifier is the primary safety mechanism in \ebpf, but it has been a major source of vulnerabilities as illustrated in~\autoref{fig:cve}.
Most \ebpf vulnerabilities stem from implementation bugs.
These bugs give adversaries an opportunity to trick the verifier into accepting a malicious kernel extension at load time. 
Nonetheless, even in the best case, where we assume that the entire \ebpf framework is bug-free, the \ebpf verifier can still be bypassed.
This is because the \ebpf verifier essentially works as a blocklist of prohibited behaviors, rejecting \ebpf programs that might not be safe to execute within the kernel.
For the \ebpf verifier to work as intended, all possible attacks must be considered ahead of time and effectively blocked.
Given the complex internals of a program, this is difficult to achieve.
For example, the \ebpf verifier used to neglect alignment checks for stack pointers.
This specification bug could corrupt spilled registers, potentially allowing adversaries to perform a denial-of-service attack~\cite{stack_dos_cve}.

To summarize, the \ebpf verifier is not entirely reliable, but the \ebpf framework trusts primarily the verifier for the safety of \ebpf programs.
Existing \ebpf CVEs have shown that relying on static verification alone could still lead to violations at runtime.
Consequently, despite their potential, the Linux community has dismissed unprivileged \ebpf programs as an unsafe feature that should not be used or expanded upon.
This motivates the need for dynamic sandboxing to strengthen the safety assurance of \ebpf programs and allow flexible kernel extensibility.


\subsection{Motivating Examples}
\label{sec:background:motivation}
We use a CVE to demonstrate the runtime violations that static verification fails to prevent, hence motivating the need for dynamic sandboxing in \ebpf.

\smallskip
\noindgras{CVE-2021-3490~\cite{cve-2021-3490}.}
A bounds tracking bug in the \ebpf verifier incorrectly tracks the bounds for 32-bit bitwise operations, leading to an out-of-bounds access vulnerability. 
In particular, the bug allows adversaries to craft a register with bounds  \texttt{u32\_min\_value} = 1 and  \texttt{u32\_max\_value}~=~0 during verification.
The verifier marks a register with bounds \texttt{u32\_min\_value} $>$ \texttt{u32\_max\_value} as containing an unknown scalar value.
When adding an unknown scalar value to a pointer register, the pointer register changes to a scalar.
Since the verifier assumes that a scalar is not a pointer, this can be exploited to leak kernel pointers to the user space.
Existing work~\cite{chompie_exploit} has exploited this bug to perform out-of-bounds read and write.
The arbitrary read access can be used to find the \texttt{cred} structure, after which the arbitrary write access is used to overwrite it to escalate privilege.
\system instruments all read and write instructions in \ebpf programs, adding dynamic checks to ensure that all memory accesses fall within the address space of an \ebpf program at runtime.
In~\S\ref{sec:evaluation:security}, we demonstrate the efficacy of \system in preventing this class of out-of-bounds access vulnerabilities.



==> eval-size.tex <==
\subsection{Size}
\label{sec:evaluation:size}

\input{table/size_overhead}
\input{table/instrumentation}

We use bpftool~\cite{bpftool} to measure the size of two \ebpf applications:
(1) The \emph{socket filter} program monitors packets by attaching to the \texttt{sock\_queue\_rcv\_skb()} function. It exchanges packet information with a user space process through an \ebpf ring buffer, and writes packet information to the standard output.
(2) the \emph{xdp} program logs the size of each ingress packet entering a networking device, and finally passes the packet back to the kernel’s networking stack.
\notesyl{do we want to talk about katran? we're not measuring its overhead but the instrumentation bit is worth discussing}

\autoref{tab:size-overhead} shows the size of JIT-compiled \ebpf images in bytes.
We observe a 115\% and 157\% increase in the size of \emph{socket filter} and \emph{xdp} \ebpf images. 
This corresponds to the number of checks we insert into the sandboxed \ebpf program during JIT compilation, as illustrated in~\autoref{tab:instrumentation}.
However, neither the size of \ebpf image nor the number of instrumentation can be used as a performance indicator.
This is because depending to the execution path, the number of checks executed at runtime might be less than that inserted into \ebpf programs.
This observation is especially common in a more complicated, real-world \ebpf application.
For instance, less than 10\% of the checks inserted into the Katran load balancer~\cite{katran} are actually executed at runtime. 


==> introduction.tex <==
\notetp{You need to fit abstract + intro on the title page for a workshop paper.}

The extended Berkeley Packet Filter (\ebpf) %
allows users to extend the Linux kernel's capabilities 
without modifying its source code.
To ensure safe extension of the kernel,
\ebpf uses a verifier to
\emph{statically} validate
access of an \ebpf program
to only an allowlist 
of functions in the kernel. \notetp{It does more than just that.}
Unfortunately,
there exist known vulnerabilities in \ebpf
that can violate kernel isolation \emph{at runtime}
and circumvent the verifier
to access arbitrary kernel memory~\cite{cve-2021-3490,cve-2020-8835} 
or execute arbitrary kernel code~\cite{cve-2021-29154}.
As a result, 
most Linux distributions~\cite{unpriv_suse,unpriv_ubuntu} allow 
\emph{only privileged users} 
to run \ebpf programs,
but doing so severely limits
\emph{unprivileged users} from exploring
the potential of \ebpf.
For example,
unprivileged containers
cannot use \ebpf 
to \eg monitor events in the host kernel. \notetp{I would suggest citing a few interesting use cases here (very short).}



\notetp{We only do SFI here. What we want to say is verifier was picked as technology due to the relatively low performance cost. However, due to the kernel complexity it is not working. We want to demonstrate that simple SFI techniques can be leveraged to prevent relevant classes of vulnerabilities.
SFI is a purely software approach and we envision possible future improvement through hardware support.
The overhead reported in this work should be seen as an upper bound demonstrating that dynamic is not only desirable from a functionality perspective, but also realistic in term of performance.}
In this work,
we propose \system,
a \emph{dynamic sandboxing} mechanism
that enforces run-time isolation
between an \ebpf program and the kernel
to confine the impact of any vulnerability
within the \ebpf program itself.
We explore a variety of kernel isolation techniques, 
including software fault isolation (SFI)~\cite{erlingsson2006xfi,castro2009fast,mao2011software},
virtualization~\cite{nikolaev2013virtuos,narayanan2019lxds,narayanan2020lightweight, proskurin2020xmp},
and hardware-assisted isolation~\cite{mckee2022preventing}, 
to protect the confidentiality and integrity 
of kernel memory from potentially malicious \ebpf programs. 
To understand the trade-offs 
between \emph{performance} and \emph{security} 
when using a particular kernel isolation technique
to sandbox an \ebpf program,
we perform comprehensive evaluations 
on \emph{all} the techniques.
More importantly,
we show that state-of-the-art 
kernel isolation mechanisms~\cite{narayanan2020lightweight,mckee2022preventing}
incur reasonably low overhead.

\begin{figure}
	\centering
	\includegraphics[width=0.9\columnwidth]{img/cve.png}
	\caption{A summary of eBPF CVEs from 2010 to 2022; 48 CVEs in  total.}
	\label{fig:cve}
\end{figure}
 
\notetp{Move discussion about relaxation of restiction to the first paragraph, cut the rest.}
We envision \system to bring many benefits besides preventing runtime violations of \ebpf programs.
Since there are overlaps between the isolation mechanism and the verifier, we see possibilities in replacing some verifier checks (e.g., memory access and control-flow integrity checks) with kernel isolation techniques. 
As shown in~\autoref{fig:cve}, the \ebpf verifier is the most significant source of vulnerabilities.
\system can reduce the size of the \ebpf verifier, potentially making its formal verification feasible and hence strengthening verifier's assurance on the safety of \ebpf programs.
With \system providing high isolation assurance between \ebpf programs and the kernel, we also hope to increase the community's confidence in unprivileged \ebpf.
We believe unprivileged \ebpf has many potential use cases should its restrictions be relaxed (\eg lift the unprivileged \ebpf ban on commodity Linux distributions).
For example, unprivileged containers could benefit from existing work that leverages \ebpf for user-defined audit logging~\cite{lim2021secure}, scheduling~\cite{kaffes2021syrup}, or synchronization~\cite{park2022application}.


\notetp{You need to review the literature. Check in particular the people organizing the workshop and on the PC. Be sure you don't miss anything.}
The dynamic sandboxing of \ebpf programs has not been explored in existing literature; rather, previous work on hardening \ebpf focuses on improving the static verifier via fuzzing~\cite{ebpf_fuzz} and formal verification~\cite{nelsonverifier} but neither enforces isolation dynamically.
On the other hand, existing work on dynamic kernel sandboxing focuses primarily on device drivers~\cite{swift2003improving, erlingsson2006xfi, ganapathy2007microdrivers, renzelmann2009decaf, castro2009fast, mao2011software}.
Although \ebpf programs and device drivers are both kernel extensions, the latter faces more challenges in terms of identifying the isolation boundary between a sandboxed component and the kernel.
This is because device drivers have unrestricted access to kernel resources, resulting in a complex driver-kernel dependency that is difficult to resolve~\cite{huang2022ksplit}. 
This can potentially lead to an over-estimation of shared resources between a sandboxed driver and the kernel~\cite{ganapathy2007microdrivers, renzelmann2009decaf}, which inevitably impacts kernel performance (e.g., due to unnecessary synchronization across the sandbox)~\cite{huang2022ksplit}.
On the contrary, \ebpf programs can only access a predefined set of kernel resources via a well-defined interface.
Instead of directly porting device driver sandboxing mechanisms to \ebpf, we leverage this knowledge to decompose an \ebpf program into an isolated compartment with minimal performance and engineering~overhead.

\noindent To summarize, we make the following contributions:
\begin{itemize}
	\item We study safety mechanisms in \ebpf and highlight its fundamental weakness --- \emph{lack of dynamic isolation} (\S\ref{sec:background}).
	\item We propose a new \ebpf dynamic sandboxing mechanism that implements software-, virtualization- and hardware-based isolation techniques configurable during kernel compilation~(\S\ref{sec:design}).
	\item We provide a comprehensive comparison of state-of-the-art kernel isolation techniques from the perspective of security and performance (\S\ref{sec:evaluation}).
\end{itemize}


==> sfi_code.tex <==

\begin{figure*}[]
	\centering
	\noindent
	\begin{subfigure}{0.25\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{img/sfi_layout.png}
		\caption{\ebpf memory layout.}
		\label{fig:sfi_layout}
	\end{subfigure}%
	\begin{subfigure}{0.35\textwidth}
		\begin{lstlisting}[language={[x86masm]Assembler},gobble=5,numbers=left,frame=tb]
			; write to %
			mov %
				
						
			; jump outside of the eBPF program
			call 0xffffffff81ac9fa0 <bpf_helper>
		\end{lstlisting}%
		\caption{Before instrumentation.}
		\label{lst:before}
	\end{subfigure}%
	\begin{subfigure}{0.36\textwidth}
		\begin{lstlisting}[language={[x86masm]Assembler},gobble=5,numbers=left,frame=tb]
			; mask write instruction 
			; (same applies to read instruction)
			push %
			lea -0x8(rbp), %
			and -0x18(%
			or  -0x10(%
			sub $0xfffffffffffffff8, %
			mov %
			pop %
			mov %
			
			; redirect call to trampoline
			mov 0xffffffff81ac9fa0, %
			callq 0xffffffffeec32b18 <trampoline>
		\end{lstlisting}%
		\caption{After instrumentation.}
		\label{lst:after}
	\end{subfigure}%
	\caption{SFI design. Each \ebpf program is loaded into its own domain, which is a logically separate portion of the kernel address space. Code transformation for enforcing address masking and trapping control transfers to a trampoline is achieved via instrumentation at the machine code level. All assembly code follows AT\&T syntax.}
	\label{fig:sfi_checks}
\end{figure*}

==> table/size_overhead.tex <==
\begin{table}[]
	\resizebox{0.8\columnwidth}{!}{%
		\begin{tabular}{l|ccc}
			\multicolumn{1}{l|}{Program} & Vanilla & Sandboxed & Overhead \\ \hline
			XDP              	& 49   	 & 126     & 157~\%  \\
			Socket Filter       & 403    & 865     & 115~\% 
		\end{tabular}%
	}
	\caption{Size of eBPF program measured in bytes.}
	\label{tab:size-overhead}
\end{table}
